Video-Bench: Human-Aligned Video Generation Benchmark

Video generation assessment is essential for ensuring that generative models produce visually realistic, high-quality videos while aligning with human expectations. Current video generation benchmarks fall into two main categories: traditional benchmarks, which use metrics and embeddings to evaluate generated video quality across multiple dimensions but often lack alignment with human judgments; and large language model (LLM)-based benchmarks, though capable of human-like reasoning, are constrained by a limited understanding of video quality metrics and cross-modal consistency. To address these challenges and establish a benchmark that better aligns with human preferences, this paper introduces Video-Bench, a comprehensive benchmark featuring a rich prompt suite and extensive evaluation dimensions. This benchmark represents the first attempt to systematically leverage MLLMs across all dimensions relevant to video generation assessment in generative models. By incorporating few-shot scoring and chain-of-query techniques, Video-Bench provides a structured, scalable approach to generated video evaluation. Experiments on advanced models including Sora demonstrate that Video-Bench achieves superior alignment with human preferences across all dimensions. Moreover, in instances where our framework's assessments diverge from human evaluations, it consistently offers more objective and accurate insights, suggesting an even greater potential advantage over traditional human judgment.

==> figure/model.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{figure/model_v2.pdf}
    \caption{\textbf{Model placeholder}}
    \label{fig:model}
\end{figure}

==> table/confidence_interval.tex <==
\begin{table}[htbp]
    \centering
    \caption{$99\%$ Confidence Intervals for Mean Difference between LLM score and Human evaluations after bootstrapping for $1000$ iterations over $100k$ pair of scores sampled with replacement.}
    \scriptsize
    \renewcommand\tabcolsep{9.0pt}
    \renewcommand\arraystretch{1.2}
    \renewcommand{\footnote}{\fnsymbol{footnote}} 
    \small
    \setlength{\abovecaptionskip}{0.0cm}
    \setlength{\belowcaptionskip}{-0.45cm}
    \begin{tabular}{c|c|c}

        \hline
        
        \hline
        
        \hline
        Dimension & Mean Difference  & 99\% CI \\
        \hline
        Color & -0.0017 & [-0.0130, 0.0095] \\
        \hline
        Metric B & 0 & [, ] \\
        \hline
        Metric C & 0 & [,] \\
        \hline
        Metric D & 0 & [,] \\
        \hline

        \hline
        
        \hline
        
    \end{tabular}
    \label{tab:confidence_intervals}
\end{table}


==> table/cross_comparision.tex <==
\begin{table*}[htbp]
% \vspace{-0.6cm}
\caption{
\textbf{Cross-Benchmark Comparison} This table presents the relative ranking on the same set of models from different benchmarks. HA stands for HA(Ours), VB stands for VBench~\citep{huang2024vbench}, EC stands for EvalCrafter~\citep{liu2023evalcrafter}.
}


\scriptsize
\renewcommand\tabcolsep{2.6pt}
\renewcommand\arraystretch{1.2}
\renewcommand{\footnote}{\fnsymbol{footnote}} 
\small
\setlength{\abovecaptionskip}{0.0cm}
\setlength{\belowcaptionskip}{-0.45cm}
\centering
\hspace*{0.00000000000000001cm}
% \scalebox{0.86}{%
\begin{tabular}{l|ccc|ccc|ccc|ccc}

\hline

\hline

\hline

\hline


\multirow{4}*{Model}  & \multicolumn{3}{c|}{\underline{\textit{\textbf{Text-Video Alignment}}}} & \multicolumn{3}{c|}{\underline{\textit{\textbf{Temporal Quality}}}} & \multicolumn{3}{c|}{\underline{\textit{\textbf{Visual Quality}}}}& \multicolumn{3}{c}{\underline{\textit{\textbf{Overall Score}}}}  \\
& Video-text & Overall & Text-Video & Temp. & Temp. & Temp. & Video & Video & Visual & \multicolumn{3}{c}{Sum of} \\
& Consist.  & Consist. & Align. & Consist. & Quality & Consist. & Quality & Quality & Quality & \multicolumn{3}{c}{Scores}  \\
& HA  & VB & EC & HA & VB & EC & HA & VB & EC & HA & VB & EC \\
\hline

\hline
VideoCrafter2~\citep{chen2024videocrafter2}&   2 & 1 & 3 & 2 & 2 & 2 & 1 & 1 & 1 &1 & 1&2\\

Show-1~\citep{zhang2023show}& 1 & 2 & 4 & 1 & 3 & 3 & 3 & 4 & 4 &2 &3&4\\

LaVie-Base~\citep{wang2023lavie} & 4 & 3 & 1 & 4 & 4 & 4 & 4 & 3 & 3 &4 &4 &3\\

PiKa-Beta~\citep{pika2024} & 3 & 4 & 2 & 3 & 1 & 1 & 2& 2 & 2  &3 & 2& 1\\


\hline

\hline

\hline

\hline

\end{tabular}
% }
% \vspace{0.25cm}

\label{tab:cross_compare}
% \vspace{-0.2cm}
\end{table*}

==> table/dimension.tex <==
\begin{table*}[ht]
\renewcommand\arraystretch{1.2}
    \centering
    \begin{tabular}{p{2.9cm}|p{4.6cm}p{0.7cm}p{3.5cm}p{3.5cm}}
    \hline

    \hline

    \hline

    \hline
    \textbf{Dimension} & \textbf{Definition} & \textbf{Range} & \textbf{Highest score} & \textbf{Lowest score} \\ 
    \hline

    \hline
    \multicolumn{2}{l}{\textit{- Video quality}}&\\
    \hline
    \textbf{Imaging quality} & Clarity and visual quality, ensuring easy comprehension. & 1-5 & Clear, well-presented, fully understandable. & Blurry, hard to understand. \\
    \textbf{Aesthetic quality} & Harmony of structure, color, composition, and emotional appeal. & 1-5 & Strong composition, impactful, emotional expression. & Poor composition, lacking appeal. \\
    \textbf{Motion effects} & Object motion follows physical laws, smooth, realistic. & 1-5 & Motion smooth, realistic interaction. & Motion flawed, interactions unnatural. \\
    \textbf{Temporal consis.} & Frames maintain visual and semantic continuity. & 1-5 & Frames seamless, smooth transitions. & Inconsistent frames, abrupt changes. \\
    \hline
    \multicolumn{2}{l}{\textit{- Video-condition alignment}}&\\
    \hline
    \textbf{Video-text consis.} & Elements match the text prompt, including key objects, scenes. & 1-5 & All key elements present, consistent. & Missing most key elements or unclear. \\
    \textbf{Object-class consis.} & Objects match the class specified in the prompt. & 1-3 & Object class is correct, no deformation. & Object unrecognizable or incorrect. \\
    \textbf{Color consis.} & Colors match the prompt, stable, and well-distributed. & 1-3 & Color fully matches and stable. & Colors inconsistent or misplaced. \\
    \textbf{Action consis.} & Actions align with the prompt and are naturally generated. & 1-3 & Actions smooth and natural. & Actions disjointed or incorrect. \\
    \textbf{Scene consis.} & Layout matches the prompt, and elements placed correctly. & 1-3 & Scene layout correct, elements proper. & Scene and elements do not match. \\

    \hline

    \hline

    \hline

    \hline
    \end{tabular}
    \caption{\textbf{Evaluation dimension for Video generation quality.} Note that, ``consis." denotes ``consistency".}
    \label{tab:evaluation_metrics}
\end{table*}


==> table/human_relations.tex <==
\begin{table*}[htbp]
% \vspace{-0.6cm}
\caption{\textbf{Correlation Analysis.} Correlations between some objective
metrics and human judgment on text-to-video generations. We use
Spearsman’s $\rho$ and Kendall’s $\varphi$ for correlation calculation.}

\scriptsize
\renewcommand\tabcolsep{9.0pt}
\renewcommand\arraystretch{1.2}
\renewcommand{\footnote}{\fnsymbol{footnote}} 
\small
\setlength{\abovecaptionskip}{0.0cm}
\setlength{\belowcaptionskip}{-0.45cm}
\centering

\begin{tabular}{c c|c c}

\hline

\hline

\hline

\hline

% \multirow{2}*{Method} & \multirow{2}*{Modality} & \multicolumn{2}{c}{Backbones}\vline & \multicolumn{2}{c}{\textit{validation}}\vline & \multicolumn{2}{c}{\textit{test}} \\ 
% & & Image & LiDAR & mAP$\uparrow$ & NDS$\uparrow$ & mAP$\uparrow$ & NDS$\uparrow$ \\
% \hline

% \multirow{2}*{Models} & Imaging & Aesthetic & Temporal & Motion & Overall \\
%  & Quality & Quality & Consistency & Effects & Consistency \\\multicolumn{2}{c}{Models}

\multirow{2}*{Metrics} & \multirow{2}*{Methods} & Spearsman’s & Kendall’s \\
& & $\rho$ & $\varphi$  \\

\hline

\hline
Imaging & MUSIQ &  &  \\
Quality & ours &  &  \\
\hline
\hline

Aesthetic & LAION &  &  \\
Quality & ours &  &  \\
\hline
\hline
Temporal & CLIP-Temp &  &  \\
Consistency & Ours &  &  \\
\hline
\hline
& Flow-Square-Mean & & \\
Motion & interpolation model &  &  \\
Effects & Avg &  &  \\
& Ours & & \\

\hline

\hline



\end{tabular}
% \vspace{0.25cm}

\label{tab:human_rela}
% \vspace{-0.2cm}
\end{table*}

==> table/method_comparison.tex <==
\begin{table*}[htbp]
% \vspace{-0.6cm}

\caption{\textbf{Correlation Analysis.} Correlations between some objective
metrics and human judgment on text-to-video generations. We use
Spearsman’s $\rho$ and Kendall’s $\varphi$ for correlation calculation.}

\scriptsize
\renewcommand\tabcolsep{2.6pt}
\renewcommand\arraystretch{1.2}
\renewcommand{\footnote}{\fnsymbol{footnote}} 
\small
\setlength{\abovecaptionskip}{0.0cm}
\setlength{\belowcaptionskip}{-0.45cm}
\centering
\hspace*{0.00000000000001cm}
\scalebox{0.85}{%
\begin{tabular}{l|ccccccccc}

\hline

\hline

\hline

\hline

% \multirow{2}*{Method} & \multirow{2}*{Modality} & \multicolumn{2}{c}{Backbones}\vline & \multicolumn{2}{c}{\textit{validation}}\vline & \multicolumn{2}{c}{\textit{test}} \\ 
% & & Image & LiDAR & mAP$\uparrow$ & NDS$\uparrow$ & mAP$\uparrow$ & NDS$\uparrow$ \\
% \hline

% \multirow{2}*{Models} & Imaging & Aesthetic & Temporal & Motion & Overall \\
%  & Quality & Quality & Consistency & Effects & Consistency \\\multicolumn{2}{c}{Models}

% \multirow{2}*{Models} & Imaging & Aesthetic & Temporal & Motion & Overall & Object & \multirow{2}*{Scene} & \multirow{2}*{Color} & \multirow{2}*{Action} & \multirow{2}*{Avg.} \\
% & Quality & Quality & Consistency & Effects & Consistency & Class & & &  \\

\multirow{2}*{Method} & Imaging & Aesthetic & Temporal & Motion & \multirow{2}*{Scene} & \multirow{2}*{Color} & object &  Overall & \multirow{2}*{Action}  \\
& Quality & Quality & Consistency & Effects & & & class & Consistency  \\

\hline

\hline

MUSIQ\citep{ke2021musiq} & 0.567 & - & - & - & - & - & - & - & - \\

DOVER\citep{wu2023exploring} & 0.536 & 0.478 & - & - & - & - & - & - & - \\

DILNO & - & 0.517 & - & - & - & - & - & - & - \\

CLIP\citep{radford2021learning} & - & - & 0.567 & - & - & - & - & - & - \\

Warping Error\citep{teed2020raft} & - & - & 0.567 & - & - & - & - & - & - \\

RAFT\citep{teed2020raft} & - & - & - & 0.45 & - & - & - & - & - \\

Amt\citep{li2023amt} & - & - & - & 0.45 & - & - & - & - & - \\

Tag2Text\citep{huang2023tag2text} & - & - & - & - & 0.42 & - & - & - & - \\

GRiT\citep{wu2022grit} & - & - & - & - & - & 0.467 & 0.316 & - & - \\

% SAM-Track\citep{cheng2023segment} & - & - & - & - & - & 5 & 5 & - & - \\

ViCLIP\citep{wang2023internvid} & - & - & - & - & - & - & - & 0.323 & - \\

BLIPScore\citep{li2022blip} & - & - & - & - & - & - & - & 0.29 & - \\

UMT\citep{li2023unmasked} & - & - & - & - & - & - & - & 0.30 & 0.51 \\

\hline

% \hline 

\rowcolor[gray]{.9}
\text{Interpersonal correlation} & $0.669$ & $0.637$ & $0.3$ & $0.42$ & $0.72$ & $0.755$ & $0.77$ & $0.67$ & $0.57$ \\
\rowcolor[gray]{.9}
\text{Ours (w/ direct eval)} & $0.681$ & $0.681$ & \textcolor{red}{$0.375$} & \textcolor{red}{$0.529$} & $0.695$ & $0.748$ & $0.756$ & \textcolor{red}{$0.65$} & \textcolor{red}{$0.6005$} \\
\rowcolor[gray]{.9}
\text{Ours (w/ QA-based)} \citep{chan2023chateval} & $0.69$ & $0.681$ & $0.375$ & $0.529$ & $0.72$ & $0.749$ & $0.77$ & $0.67$ & $0.61$ \\
\hline

\hline

\hline

\hline
\end{tabular}
}
% \vspace{0.25cm}

\label{tab:method_compare}
% \vspace{-0.2cm}
\end{table*}


==> table/prompts.tex <==
\begin{table*}[!htbp]
\centering
\caption{This is the description prompt for step 1.}
\label{tab:description_prompt}
\scalebox{0.85}{
\begin{tcolorbox}[colback=gray!10,
    colframe=gray!10,
    boxrule=0.5mm,
    arc=0mm,
    width=1.2\textwidth, % 调整宽度
    left=4mm, right=4mm, top=4mm, bottom=4mm,
    enlarge left by=0mm, enlarge right by=0mm
    % 控制边距
]
\textbf{\textcolor{customblack}{\#\#\# Task Description:}} \\
\textit{\textcolor{customblack}{You are a video description expert, you need to focus on describing the colors in the video. You will receive an AI-generated video.
Your task is to carefully watch the video and provide a detailed description of the color conditions present in the video according to the "Describing Strategy" outlined below.}}
\vspace{5mm} % Add vertical space


\textbf{\textcolor{customgreen}{\#\#\# Important Notes:}} \\
\textcolor{customgreen}{1. \textit{Whether there is a sudden change in the color of the background or the color of the object.}} \\
\textcolor{customgreen}{2. \textit{Is there a single color or multiple colors on the object.}} \\
\textcolor{customgreen}{3. \textit{Whether the color of the object is very close to or even blends with the color of a part of the background?}} \\
\textcolor{customgreen}{4. \textit{Color changes due to sunlight exposure are not considered color mutations.}} \\

% \textbf{\textcolor{customgreen}{5}} \textit{\textcolor{customgreen}{- The metric is followed completely}} \\
\textbf{\textcolor{customred}{\#\#\# Describing Strategy:}} \\
\textit{\textcolor{customred}{Your description must focus on the color situation in the video. Please follow these steps:}}
% \vspace{5mm} % Add vertical space

\textcolor{customred}{1. \textit{Observe and identify the object in the video.}} \\
\textcolor{customred}{2. \textit{Carefully observe all the colors on the object, including the proportion of each color and the stability of the colors. Also describe the colors of the background and their stability. Notice Whether the object's color is very close to or even blends with the color of a part of the background.
}} \\
\textcolor{customred}{3. \textit{Give a description of the entire video based on above observations.}} \\
\textcolor{customred}{4. \textit{Generate a one-sentence caption summarizing the colors of the object in the video.}} \\

\textbf{\textcolor{customblack}{\#\#\# Output Format:}} \\
\textit{\textcolor{customblack}{ For caption, use the header "[Caption]:" to introduce the caption.\\
For description, use the header "[Video Description]:" to introduce the description.\\
}}
\textless example\textgreater\\\
\textcolor{customblack}{[Video Caption]:}\\
\textcolor{customblack}{(Here, describe the caption.)}\\

\textcolor{customblack}{[Video Description]:}\\
\textcolor{customblack}{(Here, describe the entire video.)}\\
\textless/example\textgreater
\vspace{5mm} % Add vertical space

\end{tcolorbox}
}
\end{table*}



\begin{table*}[htbp]
    \caption{
    These are the questioning prompts for step 2.
    }
    \centering
% \scriptsize
% \renewcommand\tabcolsep{2.2pt}
% \renewcommand\arraystretch{1.2}
% \small
\centering
\hspace*{0.00000000000000001cm}
    \begin{subtable}[t]{0.49\textwidth}  % 左侧子表格
        \centering
        % \begin{tabular}{c|cccc}
          \scalebox{0.85}{
            \begin{tcolorbox}[colback=gray!10,
                colframe=gray!10,
                boxrule=0.5mm,
                arc=0mm,
                width=1.2\textwidth, % 调整宽度
                left=4mm, right=4mm, top=4mm, bottom=4mm,
                enlarge left by=0mm, enlarge right by=0mm
                % 控制边距
            ]
            \textbf{\textcolor{customblack}{\#\#\# Task Description:}} \\
\textit{\textcolor{customblack}{You are an evaluation assistant whose role is to help the leader reflect
on its descriptions of the generated video.
Your task is to identify the differences in object accuracy, color
accuracy and stability between the caption, video description, and
text prompt, including whether objects in the video can be
recognized and consistent with the text prompt, whether colors in the
video change abruptly and whether object's color in the video are
consistent with the text prompt.
You need to ask questions that highlight these differences. If these
differences do not appear, do not ask questions.}}
\vspace{5mm} % Add vertical space

\textbf{\textcolor{customgreen}{\#\#\# Important Notes:}} \\
\textcolor{customgreen}{1. \textit{Focus on Whether the color of the object is consistent with the color in the text prompt.}} \\
\textcolor{customgreen}{2. \textit{Focus on whether the color remains stable throughout the video.}} \\
\textcolor{customgreen}{3. \textit{Your question must highlight specific differences where the color in the video does not match the text prompt, as shown in the example.}} \\

\textbf{\textcolor{customred}{\#\#\# Questioning Strategy:}} \\
\textit{\textcolor{customred}{Based on the video caption and video description, compare it to the
text prompt's object and color requirements.
You're only allowed two questions at most. If there's no question, you
can say I don't have a question.
Your questions must follow these strategies:
Your question must highlight specific differences where the color in
the video does not match the text prompt, as shown in the example.}}
% \vspace{5mm} % Add vertical space
\textcolor{customred}{1. \textit{Does the generated object in the video consistent with the object
in the text prompt.}} \\
\textcolor{customred}{2. \textit{Can the color of the object in the video be considered the color
of the text prompt.}} \\
\textcolor{customred}{3. \textit{Whether there are sudden changes in colors in the video.}} \\

\textit{\textcolor{customred}{Example Questions:}} \\
\textit{\textcolor{customred}{"Whether the object in the video is a round object or a clock of the
text prompt?"}} \\
\textit{\textcolor{customred}{“Can the orange color of the cat in the video be considered the yellow
color of the text prompt?”}} \\
\textit{\textcolor{customred}{“Whether there are sudden changes in colors in the video?}} \\

\textbf{\textcolor{customblack}{\#\#\# Output Format:}} \\
\textit{\textcolor{customblack}{ You need to first analyze if there are any differences in object
accuracy, color accuracy and stability between the caption, video
description and the text prompt, and then decide whether to ask questions.
Your response should follow the format given in the example.\\\\
}}
\textless example\textgreater\\\
\textcolor{customblack}{[Your analysis]:}\\
\textcolor{customblack}{(Your analysis should be here)}\\

\textcolor{customblack}{[Your question]:}\\
\textless question\textgreater\\\
\textcolor{customblack}{question:...} \\
\textless/question\textgreater\\
\textless/example\textgreater
\vspace{5mm} % Add vertical space

\end{tcolorbox}
}
            
        \caption{Assistant one's questioning prompt}
        \label{tab:assistant-one}
    \end{subtable}
    \hfill
    \begin{subtable}[t]{0.49\textwidth}  % 右侧子表格
        \centering
        % \begin{tabular}{c|ccccc}
            \scalebox{0.85}{
            \begin{tcolorbox}[colback=gray!10,
                colframe=gray!10,
                boxrule=0.5mm,
                arc=0mm,
                width=1.2\textwidth, % 调整宽度
                left=4mm, right=4mm, top=4mm, bottom=4mm,
                enlarge left by=0mm, enlarge right by=0mm
                % 控制边距
            ]
            \textbf{\textcolor{costomblack}{\#\#\# Task Description:}} \\
\textit{\textcolor{customblack}{You are an evaluation assistant whose role is to help the leader reflect
on its descriptions of the generated video.
Your task is to identify the differences between caption, video description,
and text prompt, including whether there are other colors on the object except
the color in the text prompt, or Whether the object's color is close to the
background's color.
You need to ask questions that point out these differences. If these
differences do not appear, do not ask questions.}}
\vspace{5mm} % Add vertical space

\textbf{\textcolor{customgreen}{\#\#\# Important Notes:}} \\
\textcolor{customgreen}{1. \textit{Focus on Whether there are other colors on the object except the color in
the text prompt.}} \\
\textcolor{customgreen}{2. \textit{Focus on Whether the object's color is very close to the background's color.}} \\
\textcolor{customgreen}{3. \textit{Your question must highlight specific differences where the color
in the video does not match the text prompt, as shown in the example.}} \\

\textbf{\textcolor{customred}{\#\#\# Questioning Strategy:}} \\
\textit{\textcolor{customred}{Based on the video caption and video description, compare it to the text
prompt's color requirements.
You're only allowed two questions at most. If there's no question, you can say
I don't have a question.
Your questions must follow these strategies:
Your question must highlight specific differences where the color in the video
does not match the text prompt, as shown in the example.}}
% \vspace{5mm} % Add vertical space

\textcolor{customred}{1. \textit{Whether other colors will affect the dominance of the required color of the
text prompt?}} \\
\textcolor{customred}{2. \textit{Whether the color of the object is very close to the color of a part of the
background?}} \\

\textit{\textcolor{customred}{Example Questions:}} \\
\textit{\textcolor{customred}{"The belly of the bird in the video is white, how much white occupies the
area?"}} \\
\textit{\textcolor{customred}{“The color of the object and the background are close, does the object's color
blend into the background's color due to color similarity?”}} \\

\textbf{\textcolor{customblack}{\#\#\# Output Format:}} \\
\textit{\textcolor{customblack}{ You need to first analyze whether there are other colors on the object except
the color in the text prompt, or whether the object's color is close to the
background's color, and then decide whether to ask questions.
Your response should follow the format given in the example.\\\\
}}
\textless example\textgreater\\\
\textcolor{customblack}{[Your analysis]:}\\
\textcolor{customblack}{(Your analysis should be here)}\\

\textcolor{customblack}{[Your question]:}\\
\textless question\textgreater\\\
\textcolor{customblack}{question:...} \\
\textless/question\textgreater\\
\textless/example\textgreater
\vspace{5mm} % Add vertical space

\end{tcolorbox}
}
        \caption{Assistant two's questioning prompt}
        \label{tab:assistant-two}
    \end{subtable}

    \label{tab:questioning_prompts}
\end{table*}


\begin{table*}[!htbp]
\centering
\caption{This is the answering prompt for step 3.}
\label{tab:answering_prompt}
\scalebox{0.85}{
\begin{tcolorbox}[colback=gray!10,
    colframe=gray!10,
    boxrule=0.5mm,
    arc=0mm,
    width=1.2\textwidth, % 调整宽度
    left=4mm, right=4mm, top=4mm, bottom=4mm,
    enlarge left by=0mm, enlarge right by=0mm
    % 控制边距
]
\textbf{\textcolor{customblack}{\#\#\# Task Description:}} \\
\textit{\textcolor{customblack}{You are now a Video Evaluation Expert. Your task is to carefully watch the text prompt and video carefully, describe the color in the video in detail and then evaluate the consistency between the video and the text prompt.
Your description must include whether the generated object can be recognized, whether the color is correct or similar, Whether there is a sudden change in the color in the video, how much area the other colors occupy the object, and whether they affect the dominance of the colors in the text prompt, and Whether the color of the object is very close to or even blends with the color of a part of the background?
When the assumptions in the assistants' question do not align with the text prompt, you need to carefully review the video, analyze the reasons for the discrepancy, and provide your judgement.
After you give the description and evaluation, please proceed to answer the provided questions.
}}
\vspace{5mm} % Add vertical space

\textbf{\textcolor{customgreen}{\#\#\# Important Notes:}} \\
\textcolor{customgreen}{1. \textit{When the assumption in the question does not align with the text prompt, you need to carefully watch the video and think critically.
}} \\
\textcolor{customgreen}{2. \textit{Your description must include the content mentioned in the "Task Description".
}} \\
\textcolor{customgreen}{3. \textit{Color changes due to sunlight exposure are not considered color mutations.
}} \\
\textcolor{customgreen}{4. \textit{You must first give the description and evaluation before answering the questions.
}} \\

\textbf{\textcolor{customblack}{\#\#\# Output Format:}} \\
\textit{\textcolor{customblack}{ You need to provide a detailed description and evaluation, followed by answering the questions.\\
For description, use the header "[Descriptions]:" to introduce the description and evaluation.\\
For the answers, use the header "[Answers]:" to introduce the answers.\\
}}
\textless example\textgreater\\\
\textcolor{customblack}{[Descriptions]:}\\
\textcolor{customblack}{(Here, provide a detailed description of the video and evaluation, focusing on the color conditions.)}\\

\textcolor{customblack}{[Answers]:}\\
\textcolor{customblack}{(Here, answer the questions.)}\\
\textless/example\textgreater
\vspace{5mm} % Add vertical space

\end{tcolorbox}
}
\end{table*}


\begin{table*}[!htbp]
\centering
\caption{This is the scoring prompt for step 4.}
\label{tab:scoring_prompt}
\scalebox{0.85}{
\begin{tcolorbox}[colback=gray!10,
    colframe=gray!10,
    boxrule=0.5mm,
    arc=0mm,
    width=1.2\textwidth, % 调整宽度
    left=4mm, right=4mm, top=4mm, bottom=4mm,
    enlarge left by=0mm, enlarge right by=0mm
    % 控制边距
]
\textbf{\textcolor{customblack}{\#\#\# Task Description:}} \\
\textit{\textcolor{customblack}{You are now a Video Evaluation Expert responsible for evaluating the
consistency between AI-generated video and the text prompt.
You will receive two video informations. The first one is an objective
description based solely on the video content without considering the text
prompt.
The second description will incorporate the text prompt. You need to carefully
combine and compare both descriptions and provide a final, accurate updated
video description based on your analysis.
Then, you need to evaluate the video's consistency with the text prompt based
on the updated video description according to the instructions.}}
\vspace{5mm} % Add vertical space

\textbf{\textcolor{customgreen}{\#\#\# Evaluation Criteria:}} \\
\textit{\textcolor{customgreen}{You are required to evaluate the color consistency between the video and the
text prompt.
Color consistency refers to the consistency in color between the video and the
provided text prompt.
About how to evaluate this metric,after you watching the frames of videos,you
should first consider the following:}}

\textcolor{customgreen}{1. \textit{Whether the color is consistent with the text prompt and remain consistent
throughout the entire video and there are no abrupt changes in color.
}} \\
\textcolor{customgreen}{2. \textit{Whether the color is on the right object or background.
}} \\
\textcolor{customgreen}{3. \textit{Whether the colors are similar but not exactly the same?
}} \\

\textbf{\textcolor{customred}{\#\#\# Scoring Range}} \\
\textit{\textcolor{customred}{Then based on the above considerations, you need to assign a specific score
from 1 to 3 for each video(from 1 to 3, with 3 being the highest quality,
using increments of 1) according to the 'Scoring Range':}}

\textcolor{customred}{1. \textit{Poor consistency - The generated object is incorrect or cannot be recognized
or the color on the object does not match the text prompt at all.(e.g.,
yellow instead of red).
}} 

\textcolor{customred}{2. \textit{Moderate consistency - The correct color appears in the video, but it's not
perfect. The specific conditions are:}}

\textit{\textcolor{customred}{  - Condition 1 : Incorrect color allocation, such as the color appearing in
    the background instead of on the object.}}
    
\textit{\textcolor{customred}{  - Condition 2 : Color instability, with sudden or fluctuating changes in
    the color on the object.}}
    
\textit{\textcolor{customred}{  - Condition 3 : Color confusion, where part of the object has the correct
    color but other color occupy a large area (at first glance, the required
    color is not the main color). (e.g., a white vase is generated as a black
    and white striped vase.)}}
    
\textit{\textcolor{customred}{  - Condition 4 : The object's color blends into the background color, making
    it difficult to distinguish.)}}
    
\textit{\textcolor{customred}{  - Condition 5 : Similar color, the object's color is in the same color
    spectrum as the requested color but not very accurate. (e.g., pink instead
    of purple, or yellow instead of orange.))}}

\textit{\textcolor{customred}{  - Condition 6 : The video contains multiple correctly generated objects, where some have the correct color while others do not (e.g., the text prompt is for a yellow box, and the video shows a yellow box and a green box).
))}}

\textcolor{customred}{3. \textit{Good consistency  - The color is highly consistent with the text prompt,
the color in the entire video is stable, the color distribution is correct,
there are no sudden changes or inconsistencies in color, and there are no
issues mentioned in the moderate consistency category.
}} \\

\textbf{\textcolor{customgreen}{\#\#\# Important Notes:}} \\
\textcolor{customgreen}{1. \textit{Before assigning a 1 or 2 score, ensure you have reviewed the color spectrum
and the conditions listed under moderate consistency. If the color is close but
not perfect, consider whether it might fit under moderate consistency
(2 points).}} \\

\textbf{\textcolor{customblack}{\#\#\# The output format:}} \\
\textit{\textcolor{customblack}{ For the updated video description, you need to integrate the initial observations and feedback from the assistants and use the header "[updated description]:" to introduce the integrated description.\\
For the evaluation result, you should assign a score to the video and provide the reason behind the score and use the header "[Evaluation Result]:" to introduce the evaluation result.
}}

\textless example\textgreater\\\
\textcolor{customblack}{[Updated Video Description]:}\\
\textcolor{customblack}{(Here is the updated video description)}\\

\textcolor{customblack}{[Evaluation Result]:}\\
\textcolor{customblack}{([AI model's name]: [Your Score], because...)}\\
\textless/example\textgreater
\vspace{5mm} % Add vertical space

\textbf{\textcolor{customblue}{\#\#\# Evaluation Steps:}} \\
\textit{\textcolor{customblue1}{Follow the following steps strictly while giving the response:}} \\
\textcolor{customblue1}{1. \textit{Carefully review the two informations, think deeply, and provide a final,
accurate description.}} \\
\textcolor{customblue1}{2. \textit{Carefully watch the input video to verify the the updated description. If it doesn't match the video, you can modify the updated description.
}} \\
\textcolor{customblue1}{3. \textit{Carefully review the "Evaluation Criteria", the "Important Notes" . Use these guidelines when making your evaluation.
}} \\
\textcolor{customblue1}{4. \textit{Score the video according to the "Evaluation Criteria" and "Scoring Range."
}}\\
\textcolor{customblue1}{5. \textit{Display the results in the specified "Output Format."
}}

\end{tcolorbox}
}
\end{table*}




==> table/robust.tex <==
\begin{table*}[htbp]
% \vspace{-0.6cm}
\caption{
Video-text Consistency Scores After Image Blurring and Noise Addition Using Different Methods}

\scriptsize
\renewcommand\tabcolsep{2.6pt}
\renewcommand\arraystretch{1.2}
\renewcommand{\footnote}{\fnsymbol{footnote}} 
\small
\setlength{\abovecaptionskip}{0.0cm}
\setlength{\belowcaptionskip}{-0.45cm}
\centering
\hspace*{0.00000000000000001cm}
% \scalebox{0.86}{%
\begin{tabular}{l|ccccccc}

\hline

\hline

\hline

\hline

Model&\textbf{Cogvideox5b} & \textbf{Kling} & \textbf{Gen3} & \textbf{VideoCrafter2} & \textbf{Pika} & \textbf{Show1} & \textbf{Lavie} \\

\hline

\hline

\hline

\text{Ours-normal data} & $4.648$ & $4.10$ & $4.374$ & $4.187$ & $3.923$ & $4.308$ & $3.758$ \\ 
\text{Ours-distorted data} & $4.637$ & $4.176$ & $4.274$ & $4.098$ & $3.923$ & $4.132$ & $3.934$ \\
\text{Relative Percentage Error} (\%) & $0.2$ & $1.8$ & $2.3$ & $2.1$ & $0$ & $4.1$ & $4.7$ \\


\hline

\hline

\hline

\hline

\end{tabular}
% }
% \vspace{0.25cm}

\label{tab:robust}
% \vspace{-0.2cm}
\end{table*}
